On the Power of Weaker Pairwise Interaction: Fault-Tolerant Simulation of Population Protocols

In this paper we investigate the computational power of Population Protocols (PP) under some unreliable and/or weaker interaction models. More precisely, we focus on two features related to the power of interactions: omission failures and one-way communications. An omission failure, a notion that this paper introduces for the first time in the context of PP, is the loss by one or both parties of the information transmitted in an interaction. The failure may or may not be detected by either party. On the other hand, in one-way models, communication happens only in one direction: only one of the two agents can change its state depending on both agents' states, and the other agent may or may not be aware of the interaction. These notions can be combined, obtaining one-way protocols with (possibly detectable) omission failures. A general question is what additional power is necessary and sufficient to completely overcome the weakness of one-way protocols and enable them to simulate two-way protocols, with and without omission failures. As a basic feature, a simulator needs to implement an atomic communication of states between two agents; this task is further complicated by the anonymity of the agents, their lack of knowledge of the system, and the limited amount of memory that they may have. We provide the first answers to these questions by presenting and analyzing several simulators, i.e., wrapper protocols converting any protocol for the standard two-way model into one running on a weaker one.

==> Preliminariesshort.tex <==
% !TEX root = f_1way.tex
\subsection{Hierarchy of Models \label{sec:3}} 


\paragraph{Two-way models.}

 The model where  both starter and reactor detect an omission can be weakened by removing the detection, either on the starter's side, or on reactor's side. We obtain two symmetric models: $\delta(a_s,a_r)=\{(f_s(a_s,a_r),f_r(a_s,a_r)),\ (a_s,f_r(a_s,a_r)),\ (f_s(a_s,a_r),h(a_r)),\ (a_s,h(a_r))\},$ and \\ $\delta(a_s,a_r)=\{(f_s(a_s,a_r),f_r(a_s,a_r)),\ (o(a_s),f_r(a_s,a_r)),\  (f_s(a_s,a_r),a_r),\ (o(a_s),a_r)\}.$
If we remove the omission detection altogether, we obtain an even weaker model: $\delta(a_s,a_r)=\{(f_s(a_s,a_r),f_r(a_s,a_r)),\ (a_s,f_r(a_s,a_r)),\ (f_s(a_s,a_r),a_r)\}.$

\paragraph{One-way models.}
The interaction models that we investigate are detailed in Table~\ref{table:models}. These are essentially all possible combinations of proximity detection  and omissions on starter's and reactor's side.


Let us consider a transition function in the form $ \delta(a_s,a_r)=\{(g(a_s),f(a_s,a_r)),\ (o(a_s),h(a_r))\} $. It is easy to see that in this case the agents can simulate a model without omissions, by using the identity function for $h$ and $o$. Thus, all these models are equivalent to {\sf IT}.  Omissions are introduced by an adversary; it is clear that the adversary can avoid inserting omissions when these give more computational power, e.g., breaking symmetries.  Therefore, all models in the form $ \delta(a_s,a_r)=\{(a_s,f(a_s,a_r)),\ (o(a_s),h(a_r))\}$ (perhaps with $g$ instead of $o$ or $h$) are equivalent to {\sf IO}. These observations allow us to simplify the $15$ models of Table~\ref{table:models}, leaving only $4$ omissive models. The relationships between these models and the two-way ones are reported in Figure~\ref{figure:modcompress}.

%
%\begin{figure}[H]
%\hspace{0cm}
%    \includegraphics[scale=0.34]{figure/relat}
%      \caption{Relationships between models of Table \ref{table:models}.}
%\end{figure}

\begin{figure}[H]
\center
\includegraphics[scale=0.4]{figure/omissmap}
\caption{Relationships between omissive models. Arrows indicate the existence of trivial simulators.\label{figure:modcompress}}
\end{figure}









